A High-Performance Accelerator for Super-Resolution Processing on Embedded GPU

Recent years have witnessed impressive progress in super-resolution (SR) processing. However, its real-time inference requirement sets a challenge not only for the model design but also for the on-chip implementation. In this paper, we implement a full-stack SR acceleration framework on embedded GPU devices. The special dictionary learning algorithm used in SR models was analyzed in detail and accelerated via a novel dictionary selective strategy. Besides, the hardware programming architecture together with the model structure is analyzed to guide the optimal design of computation kernels to minimize the inference latency under the resource constraints. With these novel techniques, the communication and computation bottlenecks in the deep dictionary learning-based SR models are tackled perfectly. The experiments on the edge embedded NVIDIA NX and 2080Ti show that our method outperforms the state-of-the-art NVIDIA TensorRT significantly, and can achieve real-time performance.

==> figs/runtime-breakdown.tex <==

\pgfplotsset{
    width =0.90\linewidth,
    height=0.36\linewidth
}

\pgfplotstableread{
    Label       WG  LS  CP
    Ours        17.62  54.63  10.82
    TensorRT    78.91  54.54  10.89 
    % PyTorch     18.9548978    17.9656632  16.0842992  16.9951398
}\ggldata

\begin{tikzpicture}[scale=.94]
    % \begin{axis}[
    %             xbar stacked,
    %             xmin=0,
    %             ytick=data,
    %             yticklabels from table={\testdata}{Label}
    % ]
    \begin{axis}[
            xlabel=(ms),
            x label style={at={(axis description cs:1.10,0.15)},anchor=north},
            xbar stacked,
            xmin=-0.5,
            xmax=170,
            xtick={0, 80, 170},
            xticklabels={0, 80, 160},
            ytick=data,
            yticklabels from table={\ggldata}{Label},
            legend style={
                    cells={anchor=west},
                    legend pos=outer north east,
                },
            nodes near coords,
            nodes near coords style={/pgf/number format/.cd,precision=2},
            legend style={
                draw=none,
                at={(1.0,1.0)},
                anchor=south east,
                legend columns=4,
            }
        ]

        \addlegendentry{Dictionary}
        \addlegendentry{Conv}
        \addlegendentry{Others}

        \addplot [fill=CUlpurple] table [x=WG, meta=Label,y expr=\coordindex] {\ggldata};
        \addplot [fill=CUgold] table [x=LS, meta=Label,y expr=\coordindex] {\ggldata};
        \addplot [fill=CUribbon] table [x=CP, meta=Label,y expr=\coordindex] {\ggldata};
    \end{axis}
\end{tikzpicture}




==> pgfplot/psnr.tex <==


\pgfplotsset{
    width =0.45\textwidth,
    height=0.16\textwidth
}
    
\begin{tikzpicture}[scale=0.8]
    \begin{axis}[
        ybar,
        xmin=0.5, xmax=10.5,
        ymin=35.5, ymax=39.5,
        xticklabels={SRCNN, FSRCNN, VDSR, LapSRN, SelNet, LAPAR-A, LAPAR-A(75\%), LAPAR-A(50\%), LAPAR-A(25\%), LAPAR-A(10\%)},
        xtick={1,2,...,10},
        xtick align=inside,
        xticklabel style = {rotate=45}, %xticklabel style = {font=\tiny},
        ytick={36, 37.5, 39},
        bar width = 4pt,
        ylabel={PSNR},
        ylabel near ticks,
        legend style={
            draw=none,
            at={(0.90,1.50)},
            anchor=north,
            legend columns=3,
        }
        ]
        \addplot +[ybar, fill=myorange, draw=black, area legend]         table [x={model},  y={psnr}]     {psnr.dat};
        % \legend{}
    \end{axis}
\end{tikzpicture}

